A Real-World WebAgent with Planning, Long Context Understanding, and Program Synthesis

Pre-trained large language models (LLMs) have recently achieved better generalization and sample efficiency in autonomous web automation. However, the performance on real-world websites has still suffered from (1) open domainness, (2) limited context length, and (3) lack of inductive bias on HTML. We introduce WebAgent, an LLM-driven agent that learns from self-experience to complete tasks on real websites following natural language instructions. WebAgent plans ahead by decomposing instructions into canonical sub-instructions, summarizes long HTML documents into task-relevant snippets, and acts on websites via Python programs generated from those. We design WebAgent with Flan-U-PaLM, for grounded code generation, and HTML-T5, new pre-trained LLMs for long HTML documents using local and global attention mechanisms and a mixture of long-span denoising objectives, for planning and summarization. We empirically demonstrate that our modular recipe improves the success on real websites by over 50%, and that HTML-T5 is the best model to solve various HTML understanding tasks; achieving 18.7% higher success rate than the prior method on MiniWoB web automation benchmark, and SoTA performance on Mind2Web, an offline task planning evaluation.

==> tables/cc_html_stats.tex <==
% \begin{wraptable}{R}[0pt]{0.4\linewidth}
\begin{table}[ht]
    \begin{center}
    \begin{small}
    %\begin{sc}
    % \scalebox{0.925}{
    \scalebox{1.0}{
        \begin{tabular}{rrrr}
            \toprule
             \multirow{2}{*}{\textbf{\# of examples}} & \multicolumn{3}{c}{\textbf{\# of tokens}} \\
             \cmidrule(r){2-4}
               & \textbf{Average} & \textbf{90th} & \textbf{Max} \\
            \midrule
            3.41M & 1020 & 4566 & 7627 \\
            \bottomrule
        \end{tabular}
    }
    %\end{sc}
    \end{small}
    \end{center}
    % \vskip -0.1in
    \caption{
        Statistics of CommonCrawl HTML corpus for self-supervised denoising pre-training of HTML-T5. Input lengths are measured in tokens by~\citet{kudo2018sentencepiece}.
        }
    \label{tab:cc_html_stats}
\end{table}
%\end{wraptable}


==> tables/data_init_results.tex <==
\begin{table}[ht]
    \begin{center}
    \begin{small}
    %\begin{sc}
    \scalebox{1.0}{
        \begin{tabular}{lcrr}
            \toprule
            \textbf{CC-HTML} & \textbf{PEGASUS} & \housing{} & \textbf{MiniWoB++} \\
            \midrule
            Raw & \lyes{} & 80.56 & 56.7\% \\
            Extracted & \lno{} & 67.11 & 49.1\% \\
            % \midrule
            Extracted & \lyes{} & \textbf{82.46} & \textbf{57.0}\% \\
            \bottomrule
        \end{tabular}
    }
    %\end{sc}
    \end{small}
    \end{center}
    % \vskip -0.1in
    \caption{
        Ablations of HTML-T5-Base on dataset quality and initialization.
        We evaluate offline task planning on \housing{} and average success rate on MiniWoB with 12K dataset.
        For HTML-denoising, we prepare HTML corpus from CommonCrawl with (Extracted) or without (Raw) subtree extraction around label elements.
        We also compare the pre-training of base architectures with PEGASUS objective~\citep{zhang2020pegasus} before HTML-denoising.
        The results imply that PEGASUS pre-training is critical for the architectures and pre-processing with subtree extraction improves the downstream performance on HTML-based tasks.
        }
    \label{tab:data_init_results}
\end{table}


==> tables/descgen_results.tex <==
\begin{table*}[hb]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.875}{
\begin{tabular}{lrrrrrr}
\toprule
& \multicolumn{3}{c}{\textbf{Dev}} & \multicolumn{3}{c}{\textbf{Test}} \\
 \cmidrule(r){2-4} \cmidrule(r){5-7}
\textbf{Models} & \textbf{Accuracy} & \textbf{BLEU} & \textbf{ROUGE-1} & \textbf{Accuracy} & \textbf{BLEU} & \textbf{ROUGE-1}  \\
\midrule
LaMDA-1B~\citep{gur2022html} & 83.3 & 87.5 & 90.2 & 84.3 & 88.6 & 91.2 \\
T5-Large~\citep{gur2022html} & 83.2 & 90.2 & 90.5 & 84.3 & 91.7 & 91.5 \\
T5-XL~\citep{gur2022html} & 84.0 & 90.8 & 90.9 & 85.2 & 92.1 & 91.9 \\
\midrule
LongT5-Base & 96.4 & 98.0 & 98.5 & 95.6 & 97.4 & 98.2 \\
LongT5-Large &  98.1 & 98.9 & 99.2 & 97.7 & 98.5 & 99.0 \\
LongT5-XL & \textbf{98.4} & \textbf{99.1} & \textbf{99.3} & 98.5 & 99.2 & 99.3 \\
\midrule
HTML-T5-Base & 96.5 & 98.1 & 98.6 & 95.9 & 97.5 & 98.3 \\
HTML-T5-Large & 98.1 & 98.9 & 99.2 & 97.7 & 98.3 & 99.1 \\
HTML-T5-XL & \textbf{98.4} & 99.0 & \textbf{99.3} & \textbf{98.9} & \textbf{99.4} & \textbf{99.5} \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{
Results of Description Generation benchmark~\citep{gur2022html}. We compare LaMDA~\cite{thoppilan2022lamda}, T5, LongT5, and HTML-T5 with respect to accuracy, BLEU, and ROUGE-1 scores.
The results demonstrate that local and global attention mechanisms, shared modules between LongT5 and HTML-T5, could almost completely solve the benchmark by improving the previous best performance by over 10\%.
HTML-T5 slightly outperforms LongT5.
}
\label{tab:descgen_results}
\end{table*}


==> tables/flan_longt5.tex <==
\begin{table*}[ht]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.875}{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 & \multicolumn{2}{c}{\textbf{CoT}} & \multicolumn{2}{c}{\textbf{MMLU}} & \multicolumn{2}{c}{\textbf{BBH}} & \multicolumn{2}{c}{\textbf{BBH-CoT}} & \multicolumn{3}{c}{\textbf{Avg.}}\\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-12}
\textbf{Models} & Zero & Few  & Zero & Few & Zero & Few & Zero & Few & CoT & Direct & Total \\
\midrule
Flan-T5-Large & 35.14 & 40.03 & 40.68 & 45.12 & 25.90 & 37.48 & 26.17 & 31.45 & 33.20 & 37.29 & 35.25 \\
Flan-T5-XL & 51.74 & 52.64 & 50.76 & 52.40 & 26.09 & 40.96 & 34.12 & 35.62 & 43.53 & 42.55 & 43.04 \\
\midrule
Flan-LongT5-Large & 44.78 & 45.34 & 38.44 & 40.03 & 28.67 & 34.67 & 29.38 & 31.85 & 37.84 & 35.45 & 36.64 \\
Flan-LongT5-XL & 48.78 & 50.02 & 43.44 & 44.74 & 26.53 & 37.77 & 29.09 & 32.01 & 39.97 & 38.12 & 39.05 \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{Performance of Flan-LongT5 on reasoning tasks. We reevaluate the performance of Flan-T5~\citep{chung2022flant5}, using official checkpoints. Flan-LongT5 achieves competitive results to original Flan-T5.}
\label{tab:flan_reasoning_bench}
\end{table*}

\begin{table}[ht]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.6}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrr}
\toprule
 & \multicolumn{3}{c}{\textbf{arXiv}} & \multicolumn{3}{c}{\textbf{PubMed}} & \multicolumn{3}{c}{\textbf{BigPatent}} & \multicolumn{3}{c}{\textbf{MultiNews}} &
 \multicolumn{3}{c}{\textbf{MediaSum}} & \multicolumn{3}{c}{\textbf{CNN / Daily Mail}} \\
\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} \cmidrule(r){11-13} \cmidrule(r){14-16} \cmidrule(r){17-19}
\textbf{Models} & R-1 & R-2 & R-L & R-1 & R-2 & R-L & R-1 & R-2 & R-L & R-1 & R-2 & R-L & R-1 & R-2 & R-L & R-1 & R-2 & R-L \\
\midrule
LongT5-Large & 48.28 & 21.63 & 44.11 & 49.98 & 24.69 & 46.46 & 70.38 & 56.81 & 62.73 & 47.18 & 18.44 & 24.18 & 35.54 & 19.04 & 32.20 & 42.49 & 20.51 & 40.18 \\
LongT5-XL & 48.35 & 21.92 & 44.27 & 50.23 & 24.76 & 46.67 & \textbf{76.87} & \textbf{66.06} & \textbf{70.76} & 48.17 & 19.43 & \textbf{24.94} & 36.15 & 19.66 & 32.80 & \textbf{43.94} & \textbf{21.40} & \textbf{41.28} \\
\midrule
Flan-LongT5-Large & \textbf{48.52} & \textbf{22.00} & \textbf{44.46} & \textbf{50.46} & \textbf{25.08} & \textbf{46.96} & 70.53 & 57.13 & 63.02 & 47.76 & 18.99 & 24.52 & 35.71 & 19.18 & 32.33 & 43.13 & 20.89 & 37.28 \\
Flan-LongT5-XL & 48.37 & 21.75 & 44.22 & 50.23 & 24.75 & 46.73 & 76.31 & 65.17 & 70.01 & \textbf{48.19} & \textbf{19.47} & 24.80 & \textbf{36.16} & \textbf{19.75} & \textbf{32.81} & 43.46 & 21.00 & 37.34 \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{Performance of Flan-LongT5 on downstream summarization tasks, compared to LongT5~\citep{guo2022longt5}. We measure the performance with ROUGE-1/2/L metrics.}
\label{tab:longt5_summarization_bench}
\end{table}

==> tables/housing_flow_figure.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=1.0\linewidth]{figures/webagent_workflow.pdf}
\vskip -0.05in
\caption{
An example flow with planning, summarization, and grounded program synthesis in the \housingweb{}.
HTML-T5 iteratively predicts a decomposed sub-instruction and task-relevant snippet (\textcolor{cb_orange}{orange}) in a closed-loop manner, conditioning on the HTML documents, instruction (\textcolor{yellow}{yellow}), and history of past predictions (\textcolor{cb_green}{green}).
Flan-U-PaLM is prompted with sub-instruction and snippet (\textcolor{cb_orange}{orange}) to decode python programs (\textcolor{cb_blue}{blue}).
}
\label{fig:workflow}
\end{figure}


==> tables/housing_planning.tex <==
\begin{table}[ht]
\begin{center}
\begin{small}
\scalebox{0.9}{
\begin{tabular}{lcc}
\toprule
\textbf{Models} & \housing{} & \textbf{Diff.} \\
\midrule
LongT5-Base & 78.07 & 0.0 \\
LongT5-Large & 82.89 & 0.0 \\
LongT5-XL & 81.29 & 0.0 \\
\midrule
HTML-T5-Base & 82.46 & +4.39 \\
HTML-T5-Large & 83.63 & +0.74 \\
HTML-T5-XL & \textbf{83.92} & +2.63 \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{
Accuracy of offline evaluation on task planning.
We leverage the demonstrations in \housing{} websites.
Compared to original LongT5, and as we scale model size, HTML-T5 improves the accuracy of sub-instruction prediction.
}
\label{tab:offline_eval_results}
\end{table}


==> tables/html_t5_ablation.tex <==
\begin{table*}[t]
\begin{minipage}[c]{0.5\textwidth}
    \begin{center}
    \begin{small}
    %\begin{sc}
    \scalebox{0.825}{
        \begin{tabular}{llrr}
            \toprule
            \textbf{Architectures} & \textbf{Attention Type} & $\bm{L=2048}$ & $\bm{L=4096}$ \\
            \midrule
            Flan-T5-Base & Dense & 34.0\% & 35.3\% \\
            Long-T5-Base & Local & 43.4\% & 44.0\% \\
            Long-T5-Base & Local \& Global & \textbf{53.1}\% & \textbf{53.6}\% \\
            \bottomrule
        \end{tabular}
    }
    %\end{sc}
    \end{small}
    \end{center}
\end{minipage}
\begin{minipage}[c]{0.475\textwidth}
    \begin{center}
    \begin{small}
    %\begin{sc}
    \scalebox{0.875}{
        \begin{tabular}{lrr}
            \toprule
            \textbf{Span Length $\bm{\mu}$} &  \housing{} & \textbf{MiniWoB++} \\
            \midrule
            (no HTML-denoising) & 78.07 & 53.8\% \\
            \midrule
            3,8,64,Prefix & 80.56 & 55.2\% \\
            3,8,64 & 80.56 & 55.4\% \\
            \underline{8,64} & \textbf{82.46} & \textbf{57.0}\% \\
            8,32,64 & 82.16 & 55.6\% \\
            8,64,96 & 81.29 & 53.6\% \\
            16,64 & 79.97 & 55.2\% \\
            \bottomrule
        \end{tabular}
    }
    %\end{sc}
    \end{small}
    \end{center}
\end{minipage}
% \vskip -0.05in
\caption{
\textbf{(Left)} Architecture comparison on MiniWoB++~\cite{liu2018wge} 12K dataset with average success rate over 56 tasks. Local and global attention matches to the hierarchical tree structure of HTML, and then improves the success rate by over 15\%, compared to the instruction-finetuned dense attentions~\citep{chung2022flant5,furuta2023mmwebnav,2020t5}.
\textbf{(Right)} HTML-denoising comparison with different mixtures of span length~\citep{2020t5,tay2022ul2}.
We use LongT5-Base models for pre-training. HTML-denoising generally improves the performance on offline task planning on \housingweb{} and MiniWoB benchmark. Especially, using longer span lengths ($\mu=[8,64]$) outperforms other choices, including the default configuration in natural language domain ($\mu=[3,8,64,\text{Prefix}]$), which can reduce the less meaningful prediction from shorter spans (e.g. $\mu=3$), and inject the structural bias of HTML better.
}
\label{tab:html_t5_ablation}
\end{table*}


==> tables/html_t5_figure.tex <==
\begin{figure*}[t]
\centering
\scalebox{0.925}{
%\includegraphics[width=1.0\linewidth]{figures/html_t5_230525.pdf}
\includegraphics[width=1.0\linewidth]{figures/html_t5_230624.pdf}
}
\vskip -0.05in
\caption{
HTML-T5 consists of (1) local and global attention mechanisms~\citep{ainslie2020etc,guo2022longt5} and (2) a mixture of denoising objectives~\citep{tay2022ul2} with longer-span corruption on large-scale HTML corpus. The local and global attention mechanisms are suitable for the hierarchical tree structures of HTML documents.
Because of the sparsity of content tokens in HTML, short mean span length (e.g. $\mu=3$), often used in prior works~\citep{2020t5}, only masks less meaningful chunks. Employing longer span length (e.g. $\mu=8$) helps pre-trained language models to capture the syntax and semantics of HTML better.
We also note that this figure describes the concepts, and the elements in HTML are not always captured clearly in the attention head.
}
\label{fig:html_t5}
\end{figure*}


==> tables/miniwob_12k_sl_results.tex <==
\begin{table}[t]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.975}{
\begin{tabular}{lrr}
\toprule
\textbf{Models} & \textbf{Success Rate} & \textbf{Diff.}\\
\midrule
CC-Net~\citep{humphreys2022data} & 32.0\% & -- \\
WebT5-XL~\citep{gur2022html} & 48.4\% & -- \\
\midrule
LongT5-Base & 53.8\% & 0.0 \\
LongT5-Large & 56.3\% & 0.0 \\
LongT5-XL & 60.4\% & 0.0 \\
\midrule
Flan-LongT5-Base & 54.1\% & +0.3 \\
Flan-LongT5-Large & 56.1\% & -0.2 \\
Flan-LongT5-XL & 61.1\% & +0.7 \\
\midrule
HTML-T5-Base & 57.0\% & +3.2 \\
HTML-T5-Large & 60.8\% & +4.5 \\
HTML-T5-XL & \textbf{63.3}\% & +2.9 \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{
Average success rate of MiniWoB++ benchmark with 56 tasks. We use 12K public demonstrations~\citep{liu2018wge}, and compare HTML-T5 among supervised-finetuned baselines~\citep{humphreys2022data,gur2022html,furuta2023mmwebnav}.
HTML-T5-XL significantly outperforms WebN-T5, the prior best method, by 14.9\%, and HTML-denoising improves the performance better than instruction finetuning.
}
\label{tab:miniwob_12k_sl_results}
\end{table}



==> tables/miniwob_per_task.tex <==
\begin{table}[ht]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.825}{
\begin{tabular}{l|rr|rr}
\toprule
\textbf{Task} & \textbf{HTML-T5-XL} (347K) & \textbf{HTML-T5-XL} (12K) & \textbf{Flan-T5-XL} (347K) & \textbf{WebN-T5-XL} (12K) \\
\midrule
book-flight & 0.99 & 0.00 & 0.48 & 0.00  \\
choose-date & 0.16 & 0.03 & 0.08 & 0.00 \\
choose-date-easy & 1.00 & 0.28 & 1.00 & 0.03  \\
choose-date-medium & 0.56 & 0.14 & 0.57 & 0.00 \\
choose-list & 0.20 & 0.19 & 0.16 & 0.26  \\
click-button & 1.00 & 0.92 & 0.98 & 1.00 \\
click-button-sequence & 1.00 & 1.00 & 1.00 & 1.00  \\
click-checkboxes & 1.00 & 1.00 & 1.00 & 0.96  \\
click-checkboxes-large & 0.90 & 0.94 & 0.98 & 0.22  \\
click-checkboxes-soft & 0.99 & 0.64 & 1.00 & 0.54  \\
click-checkboxes-transfer & 1.00 & 1.00 & 0.99 & 0.63  \\
click-collapsible & 1.00 & 0.41 & 1.00 & 0.00  \\
click-collapsible-2 & 0.93 & 0.26 & 0.94 & 0.00  \\
click-color & 0.33 & 0.22 & 0.27 & 0.27  \\
click-dialog & 1.00 & 1.00 & 1.00 & 1.00  \\
click-dialog-2 & 0.74 & 0.31 & 0.34 & 0.24  \\
click-link & 0.99 & 1.00 & 1.00 & 1.00  \\
click-menu & 0.37 & 0.26 & 0.41 & 0.37  \\
click-option & 1.00 & 1.00 & 1.00 & 0.87  \\
click-pie & 0.96 & 0.89 & 0.99 & 0.51  \\
click-scroll-list & 0.00 & 0.00 & 0.00 & 0.00 \\
click-shades & 0.00 & 0.00 & 0.00 & 0.00  \\
click-shape & 0.62 & 0.57 & 0.58 & 0.53  \\
click-tab & 1.00 & 1.00 & 1.00 & 0.74  \\
click-tab-2 & 0.94 & 0.40 & 0.94 & 0.18  \\
click-tab-2-hard & 0.88 & 0.30 & 0.57 & 0.12  \\
click-test & 1.00 & 1.00 & 1.00 & 1.00  \\
click-test-2 & 1.00 & 1.00 & 1.00 & 1.00  \\
click-widget & 1.00 & 0.94 & 1.00 & 1.00  \\
count-shape & 0.67 & 0.55 & 0.64 & 0.41  \\
email-inbox & 0.94 & 0.99 & 0.99 & 0.38  \\
email-inbox-forward-nl & 1.00 & 0.92 & 1.00 & 0.60  \\
email-inbox-forward-nl-turk & 0.97 & 0.73 & 1.00 & 0.33  \\
email-inbox-nl-turk & 0.96 & 0.76 & 0.92 & 0.23 \\
enter-date & 1.00 & 0.00 & 1.00 & 0.00  \\
enter-password & 1.00 & 0.99 & 1.00 & 0.97 \\
enter-text & 1.00 & 0.96 & 1.00 & 0.89 \\
enter-text-dynamic & 1.00 & 1.00 & 1.00 & 0.98 \\
enter-time & 0.00 & 0.00 & 0.00 & 0.00 \\
focus-text & 1.00 & 1.00 & 1.00 & 1.00 \\
focus-text-2 & 1.00 & 1.00 & 1.00 & 1.00 \\
grid-coordinate & 1.00 & 1.00 & 1.00 & 0.49 \\
guess-number & 0.13 & 0.00 & 0.10 & 0.00 \\
identify-shape & 1.00 & 0.89 & 0.90 & 0.88 \\
login-user & 1.00 & 0.80 & 1.00 & 0.82 \\
login-user-popup & 1.00 & 0.63 & 0.97  & 0.72 \\
multi-layouts & 1.00 & 1.00 & 1.00  & 0.83 \\
multi-orderings & 1.00 & 1.00 & 1.00 & 0.88 \\
navigate-tree & 0.99 & 0.99 & 1.00 & 0.91 \\
search-engine & 0.93 & 0.55 & 0.59 & 0.34 \\
social-media & 0.99 & 0.93 & 0.99  & 0.21 \\
social-media-all & 0.16 & 0.78 & 0.09  & 0.00 \\
social-media-some & 0.56 & 0.53 & 0.39 & 0.02 \\
tic-tac-toe & 0.57 & 0.46 & 0.42 & 0.48 \\
use-autocomplete & 0.97 & 0.23 & 0.98 & 0.22 \\
use-spinner & 0.07 & 0.07 & 0.03 & 0.07 \\
\midrule
\textbf{Average} & \textbf{0.794} & 0.633 & 0.755 & 0.484 \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{Per-task average success rate on 56 tasks from MiniWoB++.
We refer to \citet{furuta2023mmwebnav} and \citet{gur2022html} for the baseline performances.
}
\label{tab:miniwob_per_task}
\end{table}


==> tables/miniwob_sl_results.tex <==
\begin{table}[t]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{1.0}{
\begin{tabular}{lrrr}
\toprule
\textbf{Models} & \textbf{Data} & \textbf{Success} & \textbf{Diff.}\\
\midrule
CC-Net~\citep{humphreys2022data} & 2.4M & 32.0\% & -- \\
WebN-T5-XL~\citep{gur2022html} & 12K & 48.4\% & -- \\
\midrule
LongT5-Base & \multirow{3}{*}{12K} & 53.8\% & 0.0 \\
LongT5-Large & & 56.3\% & 0.0 \\
LongT5-XL & & 60.4\% & 0.0 \\
\midrule
Flan-LongT5-Base & \multirow{3}{*}{12K} & 54.1\% & +0.3 \\
Flan-LongT5-Large & & 56.1\% & -0.2 \\
Flan-LongT5-XL & & 61.1\% & +0.7 \\
\midrule
HTML-T5-Base (ours) & \multirow{3}{*}{12K} & 57.0\% & +3.2 \\
HTML-T5-Large (ours) & & 60.8\% & +4.5 \\
HTML-T5-XL (ours) & & \textbf{63.3}\% & +2.9 \\
\midrule
Flan-T5-XL~\citep{furuta2023mmwebnav} & \multirow{2}{*}{347K} & 75.5\% & -- \\
Flan-T5-XXL~\citep{furuta2023mmwebnav} &  & 79.0\% & -- \\
\midrule
HTML-T5-XL (ours) & 347K & \textbf{79.4}\% & -- \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{
Average success rate of MiniWoB++ with 56 tasks. We use 12K demonstrations~\citep{liu2018wge}, and compare HTML-T5 among supervised-finetuned baselines~\citep{gur2022html,humphreys2022data}.
HTML-T5-XL remarkably outperforms WebN-T5-XL, the prior best method, by 14.9\%, and HTML-denoising improves the success rate better than instruction tuning.
We also finetune HTML-T5 with 347K demonstrations~\citep{furuta2023mmwebnav}, which performs better than Flan-T5-XXL (11B parameters) even with 3B parameters. See \autoref{sec:per_task_miniwob_results} for the detailed results.
}
\label{tab:miniwob_sl_results}
\end{table}



==> tables/real_html_tokens.tex <==
\begin{wrapfigure}{R}[0pt]{0.45\linewidth}
% \begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/real_html_tokens_230703.pdf}
\vskip -0.05in
\caption{
Statistics of HTML tokens among real websites.
Compared to simulator (about 500 tokens on average), HTML tokens of real websites are much longer (from 7K to 14K), which takes up the context length of large language models.
As pre-processing, we remove the irrelevant tags (e.g. \texttt{<script>}, \texttt{<meta>}) and keep necessary attributes (e.g. \texttt{id}, \texttt{type}, \texttt{value}).
}
\label{fig:real_html_tokens}
% \end{figure}
\end{wrapfigure}


==> tables/real_sim_loop.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.975\linewidth]{figures/real_sim_loop.pdf}
\vskip -0.05in
\caption{
Challenges in real-world web navigation.
Recent language model agents~\cite{furuta2023mmwebnav,gur2022html,kim2023language,yao2022react} can navigate simulated websites~\citep{shi2017miniwob,yao2022webshop}, where the agents manipulate pre-defied actions and receive simplified HTML documents that are easy to parse. In contrast, language model agents have still suffered from navigating real websites, where the agents should deal with open-ended actions, and long HTML documents that include a lot of task-irrelevant parts. Such a sim-to-real gap in web automation has been underexplored so far.
}
\label{fig:real_sim_loop}
\end{figure*}


==> tables/real_world_examples.tex <==
%% For internal version.
\begin{figure*}[t]
    \centering
    % \includegraphics[width=1.0\linewidth]{figures/real_world_examples_230922.pdf}
    \includegraphics[width=1.0\linewidth]{figures/real_world_examples_small_230922.pdf}
\vskip -0.05in
\caption{
% Example episodes of real-world web navigation in \texttt{real-estate} and \texttt{social-media} domains.
Example episodes of real-world web navigation in \texttt{map} domains.
% Considering the given instruction and HTML code, WebAgent predicts the next sub-instruction and task-relevant snippet, and then synthesizes the Python script with Selenium library, while treating the sub-instruction as a comment in the script.
}
\label{fig:real_world_examples}
\end{figure*}

%\begin{figure*}[t]
%\begin{minipage}[c]{1.0\textwidth}
%    \centering
%    \includegraphics[width=1.0\linewidth]{figures/real_world_examples.pdf}
%\end{minipage} \\
%\begin{minipage}[c]{1.0\textwidth}
%    \centering
%    \includegraphics[width=0.975\linewidth]{figures/real_sim_loop.pdf}
%\end{minipage}
%\vskip -0.05in
%\caption{
%\textbf{(Top)}
%Example traces of real-world web navigation in \texttt{real-estate} and \texttt{social-media} domains.
%\textbf{(Bottom)}
%Challenges in real-world web navigation.
%Recent language model agents~\cite{gur2022html,furuta2023mmwebnav,kim2023language,yao2022react} can navigate simulated websites~\citep{shi2017miniwob,yao2022webshop}, where the agents manipulate pre-defied actions and receive simplified HTML documents that are easy to parse. In contrast, language model agents have still suffered from navigating real websites, where the agents should deal with open-ended actions, and long HTML documents that include a lot of task-irrelevant parts.
%}
%\label{fig:real_sim_loop}
%\end{figure*}


==> tables/real_world_webnav.tex <==
\begin{table*}[t]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.875}{
\begin{tabular}{lccrrrrrrr}
\toprule
& \multicolumn{2}{c}{\textbf{HTML-T5}} & \multicolumn{2}{c}{\housing{}} & \multicolumn{2}{c}{\socialmedia{}} & \multicolumn{3}{c}{\textbf{Error Analysis}} \\
 \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-10}
 & \textbf{Plan} & \textbf{Sum} & \textbf{Success} & \textbf{Score} & \textbf{Success} & \textbf{Score} & \textbf{Program} & \textbf{Plan} & \textbf{Sum} \\
\midrule
\multirow{4}{*}{\textbf{WebAgent}} & \lno{} & \lno{} & 10\% & 55.3 & 20\% & 25.0 & 35.5\% / \underline{87.5\%} & \underline{38.7\%} / 0.0\% & 25.8\% / 12.5\% \\
 & \lyes{} & \lno{} & 50\% & 79.5 & 20\% & 38.3 & 38.9\% / \underline{65.0\%} & \underline{55.5\%} / 30.0\% & 5.6\% / 5.0\% \\
 & \lno{} & \lyes{} &  0\% & 45.7 &  25\% & 62.1 & 30.4\% / \underline{66.7\%} & \underline{39.2\%} / 13.3\% & 30.4\% / 20.0\% \\
 & \lyes{} &\lyes{} &  \textbf{65}\% & \textbf{87.6} &  \textbf{70}\% & \textbf{85.8} & 20.0\% / 33.3\% & \underline{70.0\%} / \underline{50.0\%} & 10.0\% / 16.7\% \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{
Success rate of real-world web navigation on real estate and \socialmediaweb{}.
The score stands for the percentage of covered attributes specified in given instructions.
WebAgent with HTML-T5 for planning and summarization achieves the best success (65\% on \housing{}, 70\% on \socialmedia{}), surpassing
other baselines, such as open-loop planning with prompted Flan-U-PaLM (\textbf{Plan}: \no{}) or regular-expression-based retrieval (\textbf{Sum}: \no{}).
The results imply that self-supervised experience distillation notably improve the performance, and task planning should be learned by finetuning domain language models for closed-loop planning, rather than by prompting single LLM for open-loop planning.
The error analysis describes the ratio across three types of errors in (\housing{}) / (\socialmedia{}) domains, which also points out that better adaptive planner to decompose the given instructions would contribute to further improvements of WebAgent.
}
\label{tab:realworld_results}
\end{table*}


==> tables/webagent_figure.tex <==
\begin{wrapfigure}{R}[0pt]{0.5\linewidth}
% \begin{figure}[t]
\centering
% \includegraphics[width=1.0\linewidth]{figures/WebAgent.pdf}
\includegraphics[width=1.0\linewidth]{figures/webagent_overview.pdf}
\vskip -0.05in
\caption{
WebAgent is a combination of LLMs: HTML-T5 for planning and summarization, and Flan-U-PaLM for grounded program synthesis. WebAgent can handle the bottlenecks in the real-world tasks; \textbf{open domain action space}, \textbf{complex natural language instructions}, and \textbf{long HTML pages}.
}
\label{fig:webagent}
% \end{figure}
\end{wrapfigure}

==> tables/webagent_figure_real_sim_loop.tex <==
\begin{figure*}[t]
\begin{minipage}[c]{0.6\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/real_sim_loop.pdf}
\end{minipage}
\begin{minipage}[c]{0.4\textwidth}
    \centering
    \includegraphics[width=0.975\linewidth]{figures/webagent_overview.pdf}
\end{minipage}
\vskip -0.05in
\caption{
\textbf{(Right)}
Challenges in real-world web navigation.
Recent language model agents~\cite{gur2022html,furuta2023mmwebnav,kim2023language,yao2022react} can navigate simulated websites~\citep{shi2017miniwob,yao2022webshop}, where the agents manipulate pre-defied actions and receive simplified HTML documents that are easy to parse. In contrast, language model agents have still suffered from navigating real websites, where the agents should deal with open-ended actions, and long HTML documents that include a lot of task-irrelevant parts.
\textbf{(Left)}
WebAgent is a combination of LLMs: HTML-T5 for planning and summarization, and Flan-U-PaLM for grounded program synthesis. WebAgent can handle the bottlenecks in the real-world tasks: \textbf{open domain action space}, \textbf{complex natural language instructions}, and \textbf{long HTML pages}.
}
\label{fig:webagent}
\end{figure*}


==> tables/websrc.tex <==
\begin{table}[t]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{1.0}{
\begin{tabular}{lrr}
\toprule
\textbf{Models} & \textbf{EM} & \textbf{F1} \\
\midrule
% T-PLM~\citep{chen2021websrc} & 52.12 & 61.57 \\ % BERT
% H-PLM~\citep{chen2021websrc} & 61.51 & 67.04 \\ % BERT
% V-PLM~\citep{chen2021websrc} & 62.07 & 66.66 \\ % BERT
T-PLM~\citep{chen2021websrc} & 61.67 & 69.85 \\ % ELECTRA
H-PLM~\citep{chen2021websrc} & 70.12 & 74.14 \\ % ELECTRA
V-PLM~\citep{chen2021websrc} & 73.22 & 76.16 \\ % ELECTRA
MarkupLM-Large~\citep{li2021markuplm} & 74.43 & 80.54 \\
TIE-Large~\citep{zhao2022tie} & \textbf{81.66} & \textbf{86.24} \\
\midrule
Flan-U-PaLM & 40.01 & 47.56 \\
HTML-T5-Large & 73.09 & 76.66 \\
HTML-T5-XL & 74.73 & 78.73 \\
\midrule
WebAgent & 75.50 & 85.75 \\
WebAgent (oracle) & 76.91 & \textbf{86.64} \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{
Evaluation on WebSRC~\citep{chen2021websrc} with dev set.
WebAgent, our collaborative LLMs, enhances the performance from both single generalist (Flan-U-PaLM) or specialist LLMs (HTML-T5).
WebAgent (oracle) uses oracle snippets that are guaranteed to include the answers, instead of those predicted by finetuned HTML-T5.
}
\label{tab:websrc_results}
\end{table}


==> tables/websrc_fig.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.95\linewidth]{figures/websrc_div.pdf}
\vskip -0.05in
\caption{
The performance comparison on different types of websites in WebSRC dev set.
}
\label{fig:websrc_fig}
\end{figure}


==> tables_iclr/flan_longt5.tex <==
\begin{table*}[ht]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.95}{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 & \multicolumn{2}{c}{\textbf{CoT}} & \multicolumn{2}{c}{\textbf{MMLU}} & \multicolumn{2}{c}{\textbf{BBH}} & \multicolumn{2}{c}{\textbf{BBH-CoT}} & \multicolumn{3}{c}{\textbf{Avg.}}\\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-12}
\textbf{Models} & Zero & Few  & Zero & Few & Zero & Few & Zero & Few & CoT & Direct & Total \\
\midrule
Flan-T5-Large & 35.14 & 40.03 & 40.68 & 45.12 & 25.90 & 37.48 & 26.17 & 31.45 & 33.20 & 37.29 & 35.25 \\
Flan-T5-XL & 51.74 & 52.64 & 50.76 & 52.40 & 26.09 & 40.96 & 34.12 & 35.62 & 43.53 & 42.55 & 43.04 \\
\midrule
Flan-LongT5-Large & 44.78 & 45.34 & 38.44 & 40.03 & 28.67 & 34.67 & 29.38 & 31.85 & 37.84 & 35.45 & 36.64 \\
Flan-LongT5-XL & 48.78 & 50.02 & 43.44 & 44.74 & 26.53 & 37.77 & 29.09 & 32.01 & 39.97 & 38.12 & 39.05 \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{Performance of Flan-LongT5 on reasoning tasks. We reevaluate the performance of Flan-T5~\citep{chung2022flant5}, using official checkpoints. Flan-LongT5 achieves competitive results to original Flan-T5.}
\label{tab:flan_reasoning_bench}
\end{table*}

\begin{table*}[ht]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.7}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrr}
\toprule
 & \multicolumn{3}{c}{\textbf{arXiv}} & \multicolumn{3}{c}{\textbf{PubMed}} & \multicolumn{3}{c}{\textbf{BigPatent}} & \multicolumn{3}{c}{\textbf{MultiNews}} &
 \multicolumn{3}{c}{\textbf{MediaSum}} & \multicolumn{3}{c}{\textbf{CNN / Daily Mail}} \\
\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} \cmidrule(r){11-13} \cmidrule(r){14-16} \cmidrule(r){17-19}
\textbf{Models} & R-1 & R-2 & R-L & R-1 & R-2 & R-L & R-1 & R-2 & R-L & R-1 & R-2 & R-L & R-1 & R-2 & R-L & R-1 & R-2 & R-L \\
\midrule
LongT5-Large & 48.28 & 21.63 & 44.11 & 49.98 & 24.69 & 46.46 & 70.38 & 56.81 & 62.73 & 47.18 & 18.44 & 24.18 & 35.54 & 19.04 & 32.20 & 42.49 & 20.51 & 40.18 \\
LongT5-XL & 48.35 & 21.92 & 44.27 & 50.23 & 24.76 & 46.67 & \textbf{76.87} & \textbf{66.06} & \textbf{70.76} & 48.17 & 19.43 & \textbf{24.94} & 36.15 & 19.66 & 32.80 & \textbf{43.94} & \textbf{21.40} & \textbf{41.28} \\
\midrule
Flan-LongT5-Large & \textbf{48.52} & \textbf{22.00} & \textbf{44.46} & \textbf{50.46} & \textbf{25.08} & \textbf{46.96} & 70.53 & 57.13 & 63.02 & 47.76 & 18.99 & 24.52 & 35.71 & 19.18 & 32.33 & 43.13 & 20.89 & 37.28 \\
Flan-LongT5-XL & 48.37 & 21.75 & 44.22 & 50.23 & 24.75 & 46.73 & 76.31 & 65.17 & 70.01 & \textbf{48.19} & \textbf{19.47} & 24.80 & \textbf{36.16} & \textbf{19.75} & \textbf{32.81} & 43.46 & 21.00 & 37.34 \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{Performance of Flan-LongT5 on downstream summarization tasks, compared to LongT5~\citep{guo2022longt5}. We measure the performance with ROUGE-1/2/L metrics.}
\label{tab:longt5_summarization_bench}
\end{table*}


==> tables_nature/descgen_results.tex <==
\begin{table}[hbt]
% \begin{table*}[hbt]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.65}{
\begin{tabular}{lrrrrrr}
\toprule
& \multicolumn{3}{c}{\textbf{Dev}} & \multicolumn{3}{c}{\textbf{Test}} \\
 \cmidrule(r){2-4} \cmidrule(r){5-7}
\textbf{Models} & \textbf{Accuracy} & \textbf{BLEU} & \textbf{ROUGE-1} & \textbf{Accuracy} & \textbf{BLEU} & \textbf{ROUGE-1}  \\
\midrule
LaMDA-1B~\citep{gur2022html} & 83.3 & 87.5 & 90.2 & 84.3 & 88.6 & 91.2 \\
T5-Large~\citep{gur2022html} & 83.2 & 90.2 & 90.5 & 84.3 & 91.7 & 91.5 \\
T5-XL~\citep{gur2022html} & 84.0 & 90.8 & 90.9 & 85.2 & 92.1 & 91.9 \\
\midrule
LongT5-Base & 96.4 & 98.0 & 98.5 & 95.6 & 97.4 & 98.2 \\
LongT5-Large &  98.1 & 98.9 & 99.2 & 97.7 & 98.5 & 99.0 \\
LongT5-XL & \textbf{98.4} & \textbf{99.1} & \textbf{99.3} & 98.5 & 99.2 & 99.3 \\
\midrule
HTML-T5-Base & 96.5 & 98.1 & 98.6 & 95.9 & 97.5 & 98.3 \\
HTML-T5-Large & 98.1 & 98.9 & 99.2 & 97.7 & 98.3 & 99.1 \\
HTML-T5-XL & \textbf{98.4} & 99.0 & \textbf{99.3} & \textbf{98.9} & \textbf{99.4} & \textbf{99.5} \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{
Results of Description Generation benchmark~\citep{gur2022html}. We compare LaMDA~\cite{thoppilan2022lamda}, T5, LongT5, and HTML-T5 with respect to accuracy, BLEU, and ROUGE-1 scores.
The results demonstrate that local and global attention mechanisms, shared modules between LongT5 and HTML-T5, could almost completely solve the benchmark by improving the previous best performance by over 10\%.
HTML-T5 slightly outperforms LongT5.
}
\label{tab:descgen_results}
%\end{table*}
\end{table}


==> tables_nature/housing_flow_figure.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=1.0\linewidth]{figures/webagent_workflow.pdf}
\vskip -0.05in
\caption{
An example flow with planning, summarization, and grounded program synthesis in the \housingweb{}.
HTML-T5 iteratively predicts a decomposed sub-instruction and task-relevant snippet (\textcolor{cb_orange}{orange}) in a closed-loop manner, conditioning on the HTML documents, instruction (\textcolor{yellow}{yellow}), and history of past predictions (\textcolor{cb_green}{green}).
Flan-U-PaLM is prompted with sub-instruction and snippet (\textcolor{cb_orange}{orange}) to decode python programs (\textcolor{cb_blue}{blue}).
}
\label{fig:workflow}
\end{figure*}


==> tables_nature/html_t5_ablation.tex <==
\begin{table*}[t]
\begin{minipage}[c]{0.55\textwidth}
    \begin{center}
    \begin{small}
    %\begin{sc}
    \scalebox{0.95}{
        \begin{tabular}{llrr}
            \toprule
            \textbf{Architectures} & \textbf{Attention Type} & $\bm{L=2048}$ & $\bm{L=4096}$ \\
            \midrule
            Flan-T5-Base & Dense & 34.0\% & 35.3\% \\
            Long-T5-Base & Local & 43.4\% & 44.0\% \\
            Long-T5-Base & Local \& Global & \textbf{53.1}\% & \textbf{53.6}\% \\
            \bottomrule
        \end{tabular}
    }
    %\end{sc}
    \end{small}
    \end{center}
\end{minipage}
\begin{minipage}[c]{0.45\textwidth}
    \begin{center}
    \begin{small}
    %\begin{sc}
    \scalebox{0.9}{
        \begin{tabular}{lrr}
            \toprule
            \textbf{Span Length $\bm{\mu}$} &  \housing{} & \textbf{MiniWoB++} \\
            \midrule
            (no HTML-denoising) & 78.07 & 53.8\% \\
            \midrule
            3,8,64,Prefix & 80.56 & 55.2\% \\
            3,8,64 & 80.56 & 55.4\% \\
            \underline{8,64} & \textbf{82.46} & \textbf{57.0}\% \\
            8,32,64 & 82.16 & 55.6\% \\
            8,64,96 & 81.29 & 53.6\% \\
            16,64 & 79.97 & 55.2\% \\
            \bottomrule
        \end{tabular}
    }
    %\end{sc}
    \end{small}
    \end{center}
\end{minipage}
\vskip -0.05in
\caption{
\textbf{(Left)} Architecture comparison on MiniWoB++~\cite{liu2018wge} 12K dataset with average success rate over 56 tasks. Local and global attention matches to the hierarchical tree structure of HTML, and then improves the success rate by over 15\%, compared to the instruction-finetuned dense attentions~\citep{chung2022flant5,furuta2023mmwebnav,2020t5}.
\textbf{(Right)} HTML-denoising comparison with different mixtures of span length~\citep{2020t5,tay2022ul2}.
We use LongT5-Base models for pre-training. HTML-denoising generally improves the performance on offline task planning on \housingweb{} and MiniWoB benchmark. Especially, using longer span lengths ($\mu\in\{8,6\}$) outperforms other choices, including the default configuration in natural language domain ($\mu\in\{3,8,64\}$ + Prefix LM objective), which can reduce the less meaningful prediction from shorter spans (e.g. $\mu=3$), and inject the structural bias of HTML better.
}
\label{tab:html_t5_ablation}
\end{table*}


==> tables_nature/html_t5_figure.tex <==
\begin{figure*}[t]
\centering
\scalebox{0.8}{
% \includegraphics[width=0.95\linewidth]{figures/html_t5_230624.pdf}
\includegraphics[width=0.925\linewidth]{figures/html_t5_230829.pdf}
}
\vskip -0.05in
\caption{
%\sandra{Add model inputs and outputs in this figure.}
HTML-T5 consists of (1) local and global attention mechanisms~\citep{ainslie2020etc,guo2022longt5} and (2) a mixture of denoising objectives~\citep{tay2022ul2} with longer-span corruption on large-scale HTML corpus. The local and global attention mechanisms are suitable for the hierarchical tree structures of HTML documents.
Because of the sparsity of content tokens in HTML, short mean span length (e.g. $\mu=3$), often used in prior works~\citep{2020t5}, only masks less meaningful chunks. Employing longer span length (e.g. $\mu=8$) helps pre-trained language models to capture the syntax and semantics of HTML better.
We also note that this figure describes the concepts, and the elements in HTML are not always captured clearly in the attention head.
}
\label{fig:html_t5}
\end{figure*}


==> tables_nature/miniwob_sl_results.tex <==
\begin{table}[tb]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.95}{
\begin{tabular}{lrrr}
\toprule
\textbf{Models} & \textbf{Data} & \textbf{Success} & \textbf{Diff.}\\
\midrule
CC-Net~\citep{humphreys2022data} & 2.4M & 32.0\% & -- \\
WebN-T5-XL~\citep{gur2022html} & 12K & 48.4\% & -- \\
\midrule
LongT5-Base & \multirow{3}{*}{12K} & 53.8\% & 0.0 \\
LongT5-Large & & 56.3\% & 0.0 \\
LongT5-XL & & 60.4\% & 0.0 \\
\midrule
Flan-LongT5-Base & \multirow{3}{*}{12K} & 54.1\% & +0.3 \\
Flan-LongT5-Large & & 56.1\% & -0.2 \\
Flan-LongT5-XL & & 61.1\% & +0.7 \\
\midrule
HTML-T5-Base (ours) & \multirow{3}{*}{12K} & 57.0\% & +3.2 \\
HTML-T5-Large (ours) & & 60.8\% & +4.5 \\
HTML-T5-XL (ours) & & \textbf{67.1}\% & +6.7 \\
\midrule
Flan-T5-XL~\citep{furuta2023mmwebnav} & \multirow{2}{*}{347K} & 75.5\% & -- \\
Flan-T5-XXL~\citep{furuta2023mmwebnav} &  & 79.0\% & -- \\
\midrule
HTML-T5-XL (ours) & 347K & \textbf{85.6}\% & -- \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{
Average success rate of MiniWoB++ with 56 tasks. We use 12K demonstrations~\citep{liu2018wge}, and compare HTML-T5 among supervised-finetuned baselines~\citep{gur2022html,humphreys2022data}.
HTML-T5-XL outperforms WebN-T5-XL, the prior best method, by 18.4\%. HTML-denoising yields better the success rate than instruction tuning.
Finetuned HTML-T5 with 347K demonstrations~\citep{furuta2023mmwebnav} outperforms Flan-T5-XXL (11B parameters) even with 3B parameters. See Appendix H for the detailed results.
}
\label{tab:miniwob_sl_results}
\end{table}


==> tables_nature/real_html_tokens.tex <==
% \begin{wrapfigure}{R}[0pt]{0.45\linewidth}
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{figures/real_html_tokens_230703.pdf}
\vskip -0.05in
\caption{
Statistics of HTML tokens among real websites.
Compared to simulator (about 500 tokens on average), HTML tokens of real websites are much longer (from 7K to 14K), which takes up the context length of large language models.
As pre-processing, we remove the irrelevant tags (e.g. \texttt{<script>}, \texttt{<meta>}) and keep necessary attributes (e.g. \texttt{id}, \texttt{type}, \texttt{value}).
}
\label{fig:real_html_tokens}
\end{figure}
% \end{wrapfigure}


==> tables_nature/real_sim_loop.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.925\linewidth]{figures/real_sim_loop.pdf}
\vskip -0.05in
\caption{
Challenges in real-world web automation.
Recent language model agents~\cite{furuta2023mmwebnav,gur2022html,kim2023language,yao2022react} can navigate simulated websites~\citep{shi2017miniwob,yao2022webshop}, where the agents manipulate pre-defied actions and receive simplified HTML documents that are easy to parse. In contrast, language model agents have still suffered from navigating real websites, where the agents should deal with open-ended actions, and long HTML documents that include a lot of task-irrelevant parts. Such a sim-to-real gap in web automation has been underexplored so far.
}
\label{fig:real_sim_loop}
\end{figure*}


==> tables_nature/real_world_webnav.tex <==
\begin{table*}[t]
\begin{center}
\begin{small}
%\begin{sc}
%\scalebox{0.875}{
%\begin{tabular}{lccrrrrrrr}
%\toprule
%& \multicolumn{2}{c}{\textbf{HTML-T5}} & \multicolumn{2}{c}{\housing{}} & \multicolumn{2}{c}{\socialmedia{}} & \multicolumn{3}{c}{\textbf{Error Ratio} (\%)} \\
% \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-10}
% & \textbf{Plan} & \textbf{Sum} & \textbf{Success} (\%) & \textbf{Score} (\%) & \textbf{Success} (\%) & \textbf{Score} (\%) & \textbf{Program} & \textbf{Plan} & \textbf{Sum} \\
%\midrule
%\multirow{4}{*}{\textbf{WebAgent}} & \lno{} & \lno{} & 10.0 & 55.3 & 20.0 & 25.0 & 35.5 / \underline{87.5} & \underline{38.7} / 0.0 & 25.8 / 12.5 \\
% & \lyes{} & \lno{} & 50.0 & 79.5 & 20.0 & 38.3 & 38.9 / \underline{65.0} & \underline{55.5} / 30.0 & 5.6 / 5.0 \\
% & \lno{} & \lyes{} &  0.0 & 45.7 &  25.0 & 62.1 & 30.4 / \underline{66.7} & \underline{39.2} / 13.3 & 30.4 / 20.0 \\
% & \lyes{} &\lyes{} &  \textbf{65.0} & \textbf{87.6} &  \textbf{70.0} & \textbf{85.8} & 20.0 / 33.3 & \underline{70.0} / \underline{50.0} & 10.0 / 16.7 \\
%\bottomrule
%\end{tabular}
%}
\scalebox{0.875}{
\begin{tabular}{lccrrrrrrr}
\toprule
& \multicolumn{2}{c}{\textbf{LM Modules}} & \multicolumn{2}{c}{\housing{}} & \multicolumn{2}{c}{\socialmedia{}} & \multicolumn{3}{c}{\textbf{Error Ratio} (\%)} \\
 \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-10}
 & \textbf{Plan} & \textbf{Sum} & \textbf{Success} (\%) & \textbf{Score} (\%) & \textbf{Success} (\%) & \textbf{Score} (\%) & \textbf{Program} & \textbf{Plan} & \textbf{Sum} \\
\midrule
\textbf{Flan-U-PaLM}~\citep{chung2022flant5} & \lno{} & \lno{} & 10.0 & 55.3 & 20.0 & 25.0 & 35.5 / \underline{87.5} & \underline{38.7} / 0.0 & 25.8 / 12.5 \\
\textbf{Flan-U-PaLM+P} & \lyes{} & \lno{} & 50.0 & 79.5 & 20.0 & 38.3 & 38.9 / \underline{65.0} & \underline{55.5} / 30.0 & 5.6 / 5.0 \\
\textbf{Flan-U-PaLM+S} & \lno{} & \lyes{} &  0.0 & 45.7 &  25.0 & 62.1 & 30.4 / \underline{66.7} & \underline{39.2} / 13.3 & 30.4 / 20.0 \\
\textbf{WebAgent} & \lyes{} &\lyes{} &  \textbf{65.0} & \textbf{87.6} &  \textbf{70.0} & \textbf{85.8} & 20.0 / 33.3 & \underline{70.0} / \underline{50.0} & 10.0 / 16.7 \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{
Success rate of real-world web automation on real estate and social media websites.
The score stands for the percentage of covered attributes specified in given instructions.
WebAgent, with language model modules for planning and summarization, achieves the best success (65\% on \housing{}, 70\% on \socialmedia{}), surpassing
other baselines, such as a single Flan-U-PaLM~\citep{chung2022flant5}, with a planning language model (Flan-U-PaLM+P), and with a summarization language model (Flan-U-PaLM+S).
Without language model modules, prompted Flan-U-PaLM plans in an open-loop manner (\textbf{Plan}: \no{}) and  regular-expression-based retrieval summarizes HTML inputs (\textbf{Sum}: \no{}).
The results imply that self-supervised experience distillation notably improve the performance, and task planning should be learned by finetuning domain language models for closed-loop planning, rather than by prompting single LLM for open-loop planning.
The error analysis describes the ratio across three types of errors in (\housing{}) / (\socialmedia{}) domains, which also points out that better adaptive planner to decompose the given instructions would contribute to further improvements of WebAgent.
}
\label{tab:realworld_results}
\end{table*}


==> tables_nature/webagent_figure.tex <==
% \begin{wrapfigure}{R}[0pt]{0.5\linewidth}
\begin{figure}[t]
\centering
% \includegraphics[width=1.0\linewidth]{figures/WebAgent.pdf}
% \includegraphics[width=1.0\linewidth]{figures/webagent_overview.pdf}
\includegraphics[width=1.0\linewidth]{figures/webagent_overview_230908.pdf}
\vskip -0.05in
\caption{
WebAgent is a combination of LLMs: HTML-T5 for planning and summarization, and Flan-U-PaLM for grounded program synthesis. WebAgent can handle the bottlenecks in the real-world tasks; \textbf{open domain action space}, \textbf{complex natural language instructions}, and \textbf{long HTML pages}.
}
\label{fig:webagent}
\end{figure}
% \end{wrapfigure}

==> tables_nature/websrc.tex <==
\begin{table}[t]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{1.0}{
\begin{tabular}{lrr}
\toprule
\textbf{Models} & \textbf{EM} & \textbf{F1} \\
\midrule
% T-PLM~\citep{chen2021websrc} & 52.12 & 61.57 \\ % BERT
% H-PLM~\citep{chen2021websrc} & 61.51 & 67.04 \\ % BERT
% V-PLM~\citep{chen2021websrc} & 62.07 & 66.66 \\ % BERT
T-PLM~\citep{chen2021websrc} & 61.67 & 69.85 \\ % ELECTRA
H-PLM~\citep{chen2021websrc} & 70.12 & 74.14 \\ % ELECTRA
V-PLM~\citep{chen2021websrc} & 73.22 & 76.16 \\ % ELECTRA
MarkupLM-Large~\citep{li2021markuplm} & 74.43 & 80.54 \\
TIE-Large~\citep{zhao2022tie} & \textbf{81.66} & \textbf{86.24} \\
\midrule
Flan-U-PaLM & 40.01 & 47.56 \\
HTML-T5-Large & 73.09 & 76.66 \\
HTML-T5-XL & 74.73 & 78.73 \\
\midrule
WebAgent & 75.50 & 85.75 \\
WebAgent (oracle) & 76.91 & \textbf{86.64} \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{
Evaluation on WebSRC~\citep{chen2021websrc} with dev set.
WebAgent, our collaborative LLMs, enhances the performance from both single generalist (Flan-U-PaLM) or specialist LLMs (HTML-T5).
WebAgent (oracle) uses oracle snippets that are guaranteed to include the answers, instead of those predicted by finetuned HTML-T5.
}
\label{tab:websrc_results}
\end{table}


==> tables_nature/websrc_fig.tex <==
%\begin{figure*}[ht]
\begin{figure}[ht]
\centering
\includegraphics[width=1.0\linewidth]{figures/websrc_div.pdf}
\vskip -0.05in
\caption{
The performance comparison on different types of websites in WebSRC dev set.
}
\label{fig:websrc_fig}
\end{figure}
%\end{figure*}

